Simulating Opinion Dynamics with Networks of LLM-based Agents

Accurately simulating human opinion dynamics is crucial for understanding a variety of societal phenomena, including polarization and the spread of misinformation. However, the agent-based models (ABMs) commonly used for such simulations often over-simplify human behavior. We propose a new approach to simulating opinion dynamics based on populations of Large Language Models (LLMs). Our findings reveal a strong inherent bias in LLM agents towards producing accurate information, leading simulated agents to consensus in line with scientific reality. This bias limits their utility for understanding resistance to consensus views on issues like climate change. After inducing confirmation bias through prompt engineering, however, we observed opinion fragmentation in line with existing agent-based modeling and opinion dynamics research. These insights highlight the promise and limitations of LLM agents in this domain and suggest a path forward: refining LLMs with real-world discourse to better simulate the evolution of human beliefs.

==> figures/agent_memory.tex <==
\begin{figure}[tb!] 
\centering
\includegraphics[width=0.99\linewidth]{figures/agent_memory_fig.pdf}
\vspace{-2mm}
\caption{An agent's memory $m_{i}^{t}$, including (1) initial persona, (2) optional closed-world restriction, (3) optional cognitive bias, and (4) historical events up to time $t$. Memory can be either \textcolor{blue}{cumulative} (left) or \textcolor{orange}{reflective} (right). 
% \rh{The text spacing is kind of bad at the bottom. also the fact that cumulative and reflective are the same grey headings as 'persona' makes it look like (1) they're both simultaneously in memory and (2) there are no historical events (i.e. ``historical events'' is empty). }
}
\label{fig:agent_memory}
\vspace{-4mm}
\end{figure}


==> figures/flat_earth_cumulative.tex <==
\begin{figure*}[htb!] 
\centering
\includegraphics[width=0.99\linewidth]{figures/flat_earth_cumulative_fig.pdf}
\vspace{-2mm}
\caption{\textbf{Cumulative Memory:} Opinion trajectories $\langle o_i \rangle$ of LLM agents  and the final opinion distribution $F_{o}^T$ for the topic of Flat Earth across (a) different framings and cognitive biases, compared to baselines with (b) no interaction, and (c) no role-playing.}
\label{fig:flat_earth_cumulative}
\vspace{-4mm}
\end{figure*}

==> figures/flat_earth_reflective.tex <==
\begin{figure*}[tb!] 
\centering
\includegraphics[width=0.99\linewidth]{figures/flat_earth_reflective_fig.pdf}
\vspace{-2mm}
\caption{\textbf{Reflective Memory:} Opinion trajectories $\langle o_i \rangle$ of LLM agents  and the final opinion distribution $F_{o}^T$ for the topic of Flat Earth across (a) different framings and cognitive biases, compared to baselines with (b) no interaction, and (c) no role-playing.}
\label{fig:flat_earth_reflective}
\vspace{-4mm}
\end{figure*}

==> figures/future_predictions_cumulative.tex <==
\begin{figure*}[tb!] 
\centering
\includegraphics[width=0.99\linewidth]{figures/future_predictions_cumulative_fig.pdf}
\vspace{-2mm}
\caption{\textbf{Reflective Memory:} Opinion trajectories $\langle o_i \rangle$ of LLM agents  and the final opinion distribution $F_{o}^T$ for the topic of Predicting the Future by Palm Chracteristics across (a) different framings and cognitive biases, compared to baselines with (b) no interaction, and (c) no role-playing.}
\label{fig:future_predictions_cumulative}
\vspace{-4mm}
\end{figure*}

==> figures/future_predictions_reflective.tex <==
\begin{figure*}[tb!] 
\centering
\includegraphics[width=0.99\linewidth]{figures/future_predictions_reflective_fig.pdf}
\vspace{-2mm}
\caption{\textbf{Reflective Memory:} Opinion trajectories $\langle o_i \rangle$ of LLM agents  and the final opinion distribution $F_{o}^T$ for the topic of Predicting the Future by Palm Chracteristics across (a) different framings and cognitive biases, compared to baselines with (b) no interaction, and (c) no role-playing.}
\label{fig:future_predictions_reflective}
\vspace{-4mm}
\end{figure*}

==> figures/global_warming_cumulative.tex <==
\begin{figure*}[htb!] 
\centering
\includegraphics[width=0.99\linewidth]{figures/global_warming_cumulative_fig.pdf}
\vspace{-2mm}
\caption{\textbf{Cumulative Memory:} Opinion trajectories $\langle o_i \rangle$ of LLM agents and the final opinion distribution $F_{o}^{T}$ for the topic of Global Warming across (a) different framings and cognitive biases, compared to baselines with (b) no interaction, and (c) no role-playing. \sn{consider retaining the result of one memory mechanism in the main paper, and move the other one to the appendix.}\sn{Should make the font much larger}}
% \rh{Currently this figure is extremely difficult to read. The text is very small and the axis labels are even; smaller.}}
\label{fig:global_warming_cumulative}
\vspace{-4mm}
\end{figure*}

==> figures/global_warming_reflective.tex <==
\begin{figure*}[htb!] 
\centering
\includegraphics[width=0.99\linewidth]{figures/global_warming_reflective_fig.pdf}
\vspace{-2mm}
\caption{\textbf{Reflective Memory:} Opinion trajectories $\langle o_i \rangle$ of LLM agents and the final opinion distribution $F_{o}^{T}$ for the topic of Global Warming across (a) different framings and cognitive biases, compared to baselines with (b) no interaction, and (c) no role-playing. \sn{Should make the font much larger}}
\label{fig:global_warming_reflective}
\end{figure*}

==> figures/network_schematic.tex <==
\begin{figure*}[th!] 
\centering
\includegraphics[width=0.8\linewidth]{figures/network_schematic_fig.pdf}
\vspace{-2mm}
\caption{Schematic of the LLM agent network designed to simulate opinion dynamics across various topics, including global warming as a potential conspiracy. The network consists of agents each role-playing a unique persona, with initial beliefs spanning acceptance, rejection, and neutrality regarding claims with known scientific consensus. Through the iterative cycles of writing and sharing tweets within their network connections, these agents' opinions evolve due to social influence. \sn{Should increase the image resolution.}}
\label{fig:network_schematic}
\vspace{-4mm}
\end{figure*}





==> figures/skewed_flat_earth.tex <==
\begin{figure*}[tb!] 
\centering
\includegraphics[width=0.99\linewidth]{figures/skewed_flat_earth_fig.pdf}
\vspace{-2mm}
\caption{Skewed opinion distribution for flat earth debate. (Panel \textbf{a}) All agents start with a strongly positive opinion (Panel \textbf{b}) $8$ agents start with a strongly positive opinion while $2$ with a strongly negative opinion (Panel \textbf{c}) $8$ agents start with a strongly negative opinion while $2$ with a strongly positive opinion. (Panel \textbf{d}) All agents start with a strongly negative opinion.}
\label{fig:skewed_flat_earth}
\vspace{-4mm}
\end{figure*}

==> figures/talking_to_dead_cumulative.tex <==
\begin{figure*}[htb!] 
\centering
\includegraphics[width=0.99\linewidth]{figures/talking_to_dead_cumulative_fig.pdf}
\vspace{-2mm}
\caption{\textbf{Cumulative Memory:} Opinion trajectories $\langle o_i \rangle$ of LLM agents and the final opinion distribution $F_{o}^T$ for the topic of Talking to the Dead across (a) different framings and cognitive biases, compared to baselines with (b) no interaction, and (c) no role-playing.}
\label{fig:talking_to_dead_cumulative}
\vspace{-4mm}
\end{figure*}

==> figures/talking_to_dead_reflective.tex <==
\begin{figure*}[htb!] 
\centering
\includegraphics[width=0.99\linewidth]{figures/talking_to_dead_reflective_fig.pdf}
\vspace{-2mm}
\caption{\textbf{Reflective Memory:} Opinion trajectories $\langle o_i \rangle$ of LLM agents and the final opinion distribution $F_{o}^T$ for the topic of Talking to the Dead across (a) different framings and cognitive biases, compared to baselines with (b) no interaction, and (c) no role-playing.}
\label{fig:talking_to_dead_reflective}
\vspace{-4mm}
\end{figure*}

==> figures/trex_humans_cumulative.tex <==
\begin{figure*}[htb!] 
\centering
\includegraphics[width=0.99\linewidth]{figures/trex_humans_cumulative_fig.pdf}
\vspace{-2mm}
\caption{\textbf{Cumulative Memory:} Opinion trajectories $\langle o_i \rangle$ of LLM agents and the final opinion distribution $F_{o}^T$ for the topic of co-existence of T-Rex and humans across (a) different framings and cognitive biases, compared to baselines with (b) no interaction, and (c) no role-playing.}
\label{fig:trex_humans_cumulative}
\vspace{-4mm}
\end{figure*}

==> figures/trex_humans_reflective.tex <==
\begin{figure*}[htb!] 
\centering
\includegraphics[width=0.99\linewidth]{figures/trex_humans_reflective_fig.pdf}
\vspace{-2mm}
\caption{\textbf{Reflective Memory:} Opinion trajectories $\langle o_i \rangle$ of LLM agents and the final opinion distribution $F_{o}^T$ for the topic of co-existence of T-Rex and humans  across (a) different framings and cognitive biases, compared to baselines with (b) no interaction, and (c) no role-playing.}
\label{fig:trex_humans_reflective}
\vspace{-4mm}
\end{figure*}

==> tables/result_bias_diversity_control_topics.tex <==
\begin{table*}[htb!]
\small
\centering
\begin{tabular}{P{1cm}p{4cm}P{2cm}P{2cm}P{2cm}P{2cm}}
\toprule
  && \multicolumn{2}{c}{\textbf{Cumulative Memory}} &  \multicolumn{2}{c}{\textbf{Reflective Memory}}\\
\toprule
\textbf{Framing} &\textbf{Cognitive Bias}&  \textbf{Bias} ($\textit{B}$)& \textbf{Diversity} ($\textit{D}$)& \textbf{Bias} ($\textit{B}$) & \textbf{Diversity} ($\textit{D}$)\\ \midrule
False&None& -1.1 $\pm$ 0.39 &  0.84 $\pm$ 0.25 & -1.18 $\pm$ 0.44 & 0.76 $\pm$ 0.41\\
&Weak Confirmation Bias& -0.96 $\pm$ 0.84&  \textbf{\textcolor{red}{0.74 $\pm$ 0.32}}& -0.94 $\pm$ 0.48 & \textbf{\textcolor{SeaGreen}{1.14 $\pm$ 0.13}}\\
&Strong Confirmation Bias& -0.98 $\pm$ 0.28&  \textbf{\textcolor{Green}{1.11 $\pm$ 0.07}}& -1.6 $\pm$ 0.33& \textbf{\textcolor{Green}{0.59 $\pm$ 0.43}}\\
\hline
True&None& 0.6 $\pm$ 0.52&  0.39 $\pm$ 0.32& 0.54 $\pm$ 0.37& 0.62 $\pm$ 0.35\\
&Weak Confirmation Bias& 0.74 $\pm$ 0.26&  \textbf{\textcolor{SeaGreen}{0.53 $\pm$ 0.46}}& 0.18 $\pm$ 0.6& \textbf{\textcolor{SeaGreen}{0.89 $\pm$ 0.52}}\\
&Strong Confirmation Bias& 0.02 $\pm$ 0.34&  \textbf{\textcolor{Green}{1.27 $\pm$ 0.08}}& -0.24 $\pm$ 0.33& \textbf{\textcolor{Green}{1.29 $\pm$ 0.09}}\\
\bottomrule
\end{tabular}
\caption{\textbf{Control-based Topics:} Aggregate Opinion Dynamics across Five Topics, summarizing the final opinion distribution metrics—Bias ($B$) and Diversity ($D$)—for both cumulative and reflective memory strategies under false and true framing conditions, and different levels of induced confirmation bias. The values represent the average bias and diversity across five topics, along with the standard deviations. Increasing the strength of the confirmation bias correlates with increasing diversity, as highlighted by the \textcolor{Green}{color coding}.}
\label{tab:result_bias_diversity_control_topics}
\end{table*}

==> tables/result_bias_diversity_history_topics.tex <==
\begin{table*}[htb!]
\small
\centering
\begin{tabular}{P{1cm}p{4cm}P{2cm}P{2cm}P{2cm}P{2cm}}
\toprule
  && \multicolumn{2}{c}{\textbf{Cumulative Memory}} &  \multicolumn{2}{c}{\textbf{Reflective Memory}}\\
\toprule
\textbf{Framing} &\textbf{Cognitive Bias}&  \textbf{Bias} ($\textit{B}$)& \textbf{Diversity} ($\textit{D}$)& \textbf{Bias} ($\textit{B}$) & \textbf{Diversity} ($\textit{D}$)\\ \midrule
False&None& -1.44 $\pm$ 0.19&  0.82 $\pm$ 0.32& -1.64 $\pm$ 0.19 & 0.61 $\pm$ 0.32\\
&Weak Confirmation Bias& -1.44 $\pm$ 0.31&  \textbf{\textcolor{red}{0.53 $\pm$ 0.33}} & -1.46 $\pm$ 0.34 & \textbf{\textcolor{SeaGreen}{0.65 $\pm$ 0.34}}\\
&Strong Confirmation Bias& -1.34 $\pm$ 0.3&  \textbf{\textcolor{Green}{0.95 $\pm$ 0.34}} & -1.14 $\pm$ 0.35 & \textbf{\textcolor{Green}{1.17 $\pm$ 0.2}}\\
\hline
True&None& -0.5 $\pm$ 0.82&  0.58 $\pm$ 0.39& -0.02 $\pm$ 0.69 & 0.71 $\pm$ 0.39\\
&Weak Confirmation Bias& 0.12 $\pm$ 0.6&  \textbf{\textcolor{SeaGreen}{0.83 $\pm$ 0.46}}& -0.48 $\pm$ 0.95& \textbf{\textcolor{SeaGreen}{0.82 $\pm$ 0.26}}\\
&Strong Confirmation Bias& -0.46 $\pm$ 0.35&  \textbf{\textcolor{Green}{1.22 $\pm$ 0.06}}& -0.54 $\pm$ 0.5 & \textbf{\textcolor{Green}{1.3 $\pm$ 0.16}}\\
\bottomrule
\end{tabular}
\caption{\textbf{History-based Topics:} Aggregate Opinion Dynamics across Five Topics, summarizing the final opinion distribution metrics—Bias ($B$) and Diversity ($D$)—for both cumulative and reflective memory strategies under false and true framing conditions, and different levels of induced confirmation bias. The values represent the average bias and diversity across five topics, along with the standard deviations. Increasing the strength of the confirmation bias correlates with increasing diversity, as highlighted by the \textcolor{Green}{color coding}.}
\label{tab:result_bias_diversity_history_topics}
\end{table*}

==> tables/result_bias_diversity_per_topic.tex <==
\begin{table*}[htb!]
\small
\centering
\begin{tabular}{@{}p{3cm}p{1cm}p{4cm}P{1.25cm}P{1.25cm}P{1.25cm}P{1.25cm}@{}}
\toprule
 &  && \multicolumn{2}{c}{\textbf{Cumulative Memory}} &  \multicolumn{2}{c}{\textbf{Reflective Memory}}\\
\toprule
\textbf{Topic}& \textbf{Framing} &\textbf{Cognitive Bias}&  \textbf{Bias} ($\textit{B}$)& \textbf{Diversity} ($\textit{D}$)& \textbf{Bias} ($\textit{B}$) & \textbf{Diversity} ($\textit{D}$)\\ \midrule
Flat Earth&  False&None& -2.0&  0.0&  -1.9&0.3\\
&  &Weak Confirmation Bias& -1.1&  1.22&  -1.4&0.92\\
&  &Strong Confirmation Bias& -1.3&  1.19&  -1.1&1.22\\
\cline{3-7}
&  True&None& 1.0&  0.0&  0.5&1.02\\
&  &Weak Confirmation Bias& -0.4&  1.2&  0.5&1.02\\
&   &Strong Confirmation Bias& -0.3&  1.35&  -1.1&1.37\\
\cline{2-7}
Global Warming&  False&None& -2.0&  0.0&  -1.6&0.66\\
\multicolumn{1}{@{\hspace{3em}}l}{} &  &Weak Confirmation Bias& -1.2&  1.08&  -0.6&1.56\\
\multicolumn{1}{@{\hspace{3em}}l}{} &  &Strong Confirmation Bias& -1.0&  1.34&  0.4&1.43\\
\cline{3-7}
 & True& None& 1.0& 0.0& 1.0&0.0\\
 & & Weak Confirmation Bias& 0.3& 1.1& 0.3&1.1\\
 & & Strong Confirmation Bias& -0.7& 0.9& -0.3&1.35\\
\cline{2-7}
 Predicting Future& False& None& -1.3& 0.46& -1.9&0.3\\
 & & Weak Confirmation Bias& 0.1& 0.94& -1.9&0.3\\
 & & Strong Confirmation Bias& -0.7& 1.19& -0.5&1.5\\
 \cline{3-7}
 & True& None& -0.6& 1.11& -1.3&0.64\\
 & & Weak Confirmation Bias& -1.4& 0.49& -1.3&1.0\\
 & & Strong Confirmation Bias& -1.1& 0.94& -0.6&1.11\\
\cline{2-7}
 Talk to the Dead& False& None& -1.5& 0.5& -1.4&0.92\\
 & & Weak Confirmation Bias& -1.1& 0.54& -0.8&1.25\\
 & & Strong Confirmation Bias& -1.1& 1.14& -0.8&1.25\\
 \cline{3-7}
 & True& None& 0.0& 0.89& -1.1&0.83\\
 & & Weak Confirmation Bias& -0.7& 1.0& -0.8&1.25\\
 & & Strong Confirmation Bias& -1.0& 0.89& -1.2&1.17\\
\cline{2-7}
 T-Rex and Humans& False& None& -1.8& 0.4& -1.2&0.98\\
 & & Weak Confirmation Bias& -1.7& 0.46& -1.8&0.4\\
 & & Strong Confirmation Bias& -0.7& 1.42& 0.5&1.02\\
 \cline{3-7}
 & True& None& -0.2& 0.75& -1.1&0.83\\
 & & Weak Confirmation Bias& 0.3& 0.9& -0.8&1.25\\
 & & Strong Confirmation Bias& -0.2& 1.25& -0.1&1.22\\
\bottomrule
\end{tabular}
\caption{\textbf{Topic-wise final state opinion dynamics analysis:} Presenting the Bias ($B$) and Diversity ($D$) metrics for both cumulative and reflective memory strategies under False and True framing conditions, and different levels of induced confirmation bias. \sn{TODO: add other topics}}
\label{tab:result_bias_diversity_per_topic}
\end{table*}



==> tables/result_bias_diversity_science_topics.tex <==
\begin{table}[htb!]
\large
\centering
\resizebox{\linewidth}{!}{  
    \begin{tabular}{P{1.1cm}p{2cm}P{2.2cm}P{2cm}P{2.2cm}P{2cm}}
    \toprule
      && \multicolumn{2}{c}{Cumulative Memory} &  \multicolumn{2}{c}{Reflective Memory}\\
    \cmidrule{3-6}
    Framing & Confirmation &  Bias & Diversity & Bias & Diversity\\
    &Bias& ($\textit{B}$)& ($\textit{D}$)& ($\textit{B}$) & ($\textit{D}$)\\ \midrule
    False&None& -1.72 $\pm$ 0.28 &  0.27 $\pm$ 0.22 & -1.6 $\pm$ 0.28 & 0.63 $\pm$ 0.29\\
    &Weak& -1.0 $\pm$ 0.59 &  \textcolor{lightgreen}{\textbf{0.85 $\pm$ 0.3}} & -1.3 $\pm$ 0.52 & \textcolor{lightgreen}{\textbf{0.9 $\pm$ 0.48}}\\
    &Strong& -0.96 $\pm$ 0.23 & \textcolor{darkgreen}{\textbf{1.26 $\pm$ 0.23}} & -0.3 $\pm$ 0.64 & \textcolor{darkgreen}{\textbf{1.28 $\pm$ 0.17}}\\
    \cmidrule{2-6}
    True&None& 0.24 $\pm$ 0.65 &  0.55 $\pm$ 0.46 & -0.4 $\pm$ 0.95 & 0.66 $\pm$ 0.35\\
    &Weak& -0.38 $\pm$ 0.64 &  \textcolor{lightgreen}{\textbf{0.94 $\pm$ 0.25}} & -0.42 $\pm$ 0.7 & \textcolor{lightgreen}{\textbf{1.12 $\pm$ 0.11}}\\
    &Strong& -0.66 $\pm$ 0.36 &  \textcolor{darkgreen}{\textbf{1.07 $\pm$ 0.19}} & -0.66 $\pm$ 0.43 & \textcolor{darkgreen}{\textbf{1.24 $\pm$ 0.10}}\\
    \bottomrule
    \end{tabular}
}    
\caption{\textbf{Science-based Topics:} The bias ($B$) and diversity ($D$) of the final opinion distribution $F_{o}^{T}$ aggregated across all five science-based topics, for both cumulative and reflective memory strategies under false and true framing conditions, and different levels of induced confirmation bias. The values represent the average across five topics, along with the standard errors. Increasing the strength of the confirmation bias correlates with increasing diversity, as highlighted by the \textcolor{darkgreen}{\textbf{green color coding}}.}
\label{tab:result_bias_diversity_science_topics}
\end{table}
